Jorge: Approximate Preconditioning for GPU-efficient Second-order Optimization

Despite their better convergence properties compared to first-order optimizers, second-order optimizers for deep learning have been less popular due to their significant computational costs. The primary efficiency bottleneck in such optimizers is matrix inverse calculations in the preconditioning step, which are expensive to compute on GPUs. In this paper, we introduce Jorge, a second-order optimizer that promises the best of both worlds -- rapid convergence benefits of second-order methods, and high computational efficiency typical of first-order methods. We address the primary computational bottleneck of computing matrix inverses by completely eliminating them using an approximation of the preconditioner computation. This makes Jorge extremely efficient on GPUs in terms of wall-clock time. Further, we describe an approach to determine Jorge's hyperparameters directly from a well-tuned SGD baseline, thereby significantly minimizing tuning efforts. Our empirical evaluations demonstrate the distinct advantages of using Jorge, outperforming state-of-the-art optimizers such as SGD, AdamW, and Shampoo across multiple deep learning models, both in terms of sample efficiency and wall-clock time.

==> limitations.tex <==
In this study, we evaluate Jorge against SGD, primarily due to its wide
popularity in many deep learning tasks.  Although we've shown Jorge works well
after single-shot tuning from SGD, we cannot guarantee similar results for
Adam, another popular optimizer, especially in the field of Large Language
Models.  Thus, we aim to propose a set rules and heuristics for single-shot
tuning Jorge from Adam in subsequent research.

Another goal of our subsequent research is to create a distributed Jorge.
Firstly, this would reduce memory consumption by distributing memory across
GPUs.  Jorge's memory consumption is 1.5x that of Adam without grafting, and 2x
with grafting; Adam maintains 2 buffers per parameter, Jorge maintains 3
without grafting, and 4 with.  Secondly, Jorge is implemented serially, yet
outperforms distributed Shampoo and all other serially-implemented optimizers
we tested, in terms of wall-clock time to reach a target validation accuracy.
A distributed Jorge suggests even better performance.


